Low-Carbon Economic Dispatch of Bulk Power Systems Using Nash Bargaining Game

Decarbonization of power systems plays a crucial role in achieving carbon neutral goals across the globe, but there exists a sharp contradiction between the emission reduction and levelized generation cost. Therefore, it is of great importance for power system operators to take economic as well as low-carbon factors into account. This paper establishes a low-carbon economic dispatch model of bulk power systems based on Nash bargaining game, which derives a Nash bargaining solution making a reasonable trade-off between economic and low-carbon objectives. Because the Nash bargaining solution satisfies Pareto effectiveness, we analyze the computational complexity of Pareto frontiers with parametric linear programming and interpret the inefficiency of the method. Instead, we assign a group of dynamic weights in the objective function of the proposed low-carbon economic dispatch model so as to improve the computational efficiency by decoupling time periods and avoiding the complete computation of Pareto frontiers. In the end, we validate the proposed model and the algorithm by a realistic nationwide simulation in mainland China.

==> bib_draft.tex <==
@misc{b1,
  author = {IEA},
  title = {Energy Statistics Data Browser},
  howpublished = {\url{https://www.iea.org/data-and-statistics/data-tools/energy-statistics-data-browser}},
  year = {2022}
}

@article{b2,
    title={Research on peaking carbon emissions of power sector in China and the emissions mitigation analysis(in Chinese)},
    author={Chen, Yi and Tian, Chuan and Cao, Yin and others},
    journal={Climate Change Research},
    volume={16},
    number={05},
    pages={632--640},
    year={2020}
}

@article{b3,
  title={Net-zero emissions energy systems},
  author={Davis, Steven J and Lewis, Nathan S and Shaner, Matthew and Aggarwal, Sonia and Arent, Doug and Azevedo, In{\^e}s L and Benson, Sally M and Bradley, Thomas and Brouwer, Jack and Chiang, Yet-Ming and others},
  journal={Science},
  volume={360},
  number={6396},
  pages={eaas9793},
  year={2018},
  publisher={American Association for the Advancement of Science}
}


@incollection{b4,
  title={Multi-objective optimization: classical and evolutionary approaches},
  author={Elarbi, Maha and Bechikh, Slim and Ben Said, Lamjed and Datta, Rituparna},
  booktitle={Recent advances in evolutionary multi-objective optimization},
  pages={1--30},
  year={2017},
  publisher={Springer}
}


@incollection{b5,
  title={Integrated system identification and optimization},
  author={Haimes, Yacov Y},
  booktitle={Control and Dynamic Systems},
  volume={10},
  pages={435--518},
  year={1973},
  publisher={Elsevier}
}


@article{b6,
  title={Inefficiency of Nash equilibria},
  author={Dubey, P},
  journal={Mathematics of Operations Research},
  volume={11},
  number={1},
  pages={1-8},
  year={1986}
}


@article{b7,
  author={Yang, Zhifang and Bose, Anjan and Zhong, Haiwang and Zhang, Ning and Lin, Jeremy and Xia, Qing and Kang, Chongqing},
  journal={IEEE Transactions on Power Systems}, 
  title={LMP Revisited: A Linear Model for the Loss-Embedded LMP}, 
  year={2017},
  volume={32},
  number={5},
  pages={4080-4090},
  doi={10.1109/TPWRS.2017.2648816}}


@article{b8,
author={Ji-Yuan Fan and Lan Zhang},  journal={IEEE Transactions on Power Systems},   title={Real-time economic dispatch with line flow and emission constraints using quadratic programming},   year={1998},  volume={13},  number={2},  pages={320-325},  doi={10.1109/59.667345}}


@article{b9,
title = {Emissions impacts of using energy storage for power system reserves},
journal = {Applied Energy},
volume = {168},
pages = {444-456},
year = {2016},
issn = {0306-2619},
doi = {https://doi.org/10.1016/j.apenergy.2016.01.061},
url = {https://www.sciencedirect.com/science/article/pii/S0306261916300411},
author = {Yashen Lin and Jeremiah X. Johnson and Johanna L. Mathieu}
}


@article{b10,
title = {Impacts of CO2 emission constraints on technology selection and energy resources for power generation in Bangladesh},
journal = {Energy Policy},
volume = {39},
number = {4},
pages = {2043-2050},
year = {2011},
issn = {0301-4215},
doi = {https://doi.org/10.1016/j.enpol.2011.01.044},
url = {https://www.sciencedirect.com/science/article/pii/S0301421511000553},
author = {Md. {Alam Hossain Mondal} and Jyotirmay Mathur and Manfred Denich}
}


@article{b11,
title = {Environmental shutdown of coal-fired generators for greenhouse gas reduction: A case study of South Korea},
journal = {Applied Energy},
volume = {252},
pages = {113453},
year = {2019},
issn = {0306-2619},
doi = {https://doi.org/10.1016/j.apenergy.2019.113453},
url = {https://www.sciencedirect.com/science/article/pii/S0306261919311274},
author = {Hansol Shin and Tae Hyun Kim and Hyoungtae Kim and Sungwoo Lee and Wook Kim}
}


@article{b12,
  title={Emission constrained dynamic dispatch},
  author={ Granelli, G. P.  and  Montagna, M.  and  Pasini, G. L.  and  Marannino, P. },
  journal={Electric Power Systems Research},
  volume={24},
  number={1},
  pages={55-64},
  year={1992},
}


@article{b13,
title = {A multi-period, multi-regional generation expansion planning model incorporating unit commitment constraints},
journal = {Applied Energy},
volume = {158},
pages = {310-331},
year = {2015},
issn = {0306-2619},
doi = {https://doi.org/10.1016/j.apenergy.2015.08.054},
url = {https://www.sciencedirect.com/science/article/pii/S0306261915009873},
author = {Nikolaos E. Koltsaklis and Michael C. Georgiadis}
}


@article{b14,
  title={A low-carbon economic dispatch model incorporated with consumption-side emission penalty scheme},
  author={ Shao, C.  and  Ding, Y.  and  Wang, J. },
  journal={Applied Energy},
  volume={238},
  number={MAR.15},
  pages={1084-1092},
  year={2019},
}


@article{b15,
  title={Economic and environmental dispatch of power/CHP production systems},
  author={Peter and Brre and Eriksen},
  journal={Electric Power Systems Research},
  volume={57},
  number={1},
  pages={33-39},
  year={2001},
}


@article{b16,  author={Olsen, Daniel J. and Dvorkin, Yury and Fernández-Blanco, Ricardo and Ortega-Vazquez, Miguel A.},  journal={IEEE Transactions on Power Systems},   title={Optimal Carbon Taxes for Emissions Targets in the Electricity Sector},   year={2018},  volume={33},  number={6},  pages={5892-5901},  doi={10.1109/TPWRS.2018.2827333}}


@article{b17,  author={Wang, Yunqi and Qiu, Jing and Tao, Yuechuan and Zhao, Junhua},  journal={IEEE Transactions on Power Systems},   title={Carbon-Oriented Operational Planning in Coupled Electricity and Emission Trading Markets},   year={2020},  volume={35},  number={4},  pages={3145-3157},  doi={10.1109/TPWRS.2020.2966663}}


@article{b18,  author={Gu, Nan and Wang, Haoxiang and Zhang, Jiasheng and Wu, Chenye},  journal={IEEE Transactions on Power Systems},   title={Bridging Chance-Constrained and Robust Optimization in an Emission-Aware Economic Dispatch With Energy Storage},   year={2022},  volume={37},  number={2},  pages={1078-1090},  doi={10.1109/TPWRS.2021.3102412}}


@article{b19,
  title={Two-stage clearing model for day-ahead electricity market considering impact of carbon emissions trading markect(in Chinese)},
  author={Lu, Z and Liu, M and Shang, N and others},
  journal={Automation of Electric Power Systems},
  volume={46},
  number={10},
  pages={159-170},
  year={2022},
}


@article{b20,
  title={Medium and Long-term Power Purchase Plan Based on Bargaining Game},
  author={ Wang, Y.  and  Yuan, G.  and  Wang, C.  and  Mei, S. W.  and  Chen, L. },
  journal={Proceedings of the Chinese Society of Universities for Electric Power System and its Automation},
  year={2013},
}


@article{b21,  author={Wei, Wei and Wang, Jianhui and Mei, Shengwei},  journal={IEEE Transactions on Power Systems},   title={Convexification of the Nash Bargaining Based Environmental-Economic Dispatch},   year={2016},  volume={31},  number={6},  pages={5208-5209},  doi={10.1109/TPWRS.2016.2521322}}


@article{b22,
  title={The bargaining problem},
  author={Nash, Jr J F},
  journal={Econometrica: Journal of the Econometric Society},
  volume={},
  number={},
  pages={155-162},
  year={1950},
}


@article{b23,
  title={Geometric Algorithm for Multiparametric Linear Programming},
  author={ Borrelli, F.  and  Bemporad, A.  and  Morari, M. },
  journal={Journal of Optimization Theory and Applications},
  volume={118},
  number={3},
  pages={515-540},
  year={2003},
}


@book{b24,
  title={Optimization theory and algorithms(in Chinese)},
  author={Chen, Baolin},
  publisher={Tsinghua University Press},
  pages={143-145},
  year={2005}
}



@misc{b25,
  author = {National Renewable Energy Laboratory (NREL)},
  title = {Geospatial Data Science},
  howpublished = {\url{https://www.nrel.gov/gis/}}
}


@misc{b26,
  author = {The World Bank},
  title = {State and Trends of Carbon Pricing 2022},
  howpublished = {\url{https://openknowledge.worldbank.org/handle/10986/37455}},
  year={2022},
  month={May},
  doi={10.1596/978-1-4648-1895-0}
}



\iffalse
%下为主文档内插入参考文献的形式，被注释掉

\begin{thebibliography}{00}
%\bibitem{b1} Yuan H, Dong X, Liu Q, et al. Electricity retail side market framework design in national unified electricity market system[J/OL]. Power System Technology: 1-12[2022-09-13]. DOI:10.13335/j.1000-3673.pst.2022.0592. (in Chinese)
\bibitem{b1} IEA (2022), Energy Statistics Data Browser, IEA, Paris https://www.iea.org/data-and-statistics/data-tools/energy-statistics-data-browser
\bibitem{b2} Chen Y, Tian C, Cao Y, et al. Research on peaking carbon emissions of power sector in China and the emissions mitigation analysis[J]. Climate Change Research, 2020, 16(05): 632-640. (in Chinese)
\bibitem{b3} Steven J. Davis, et al. Net-zero Emissions Energy Systems[J]. Science,2018,360(6396).
\bibitem{b4} Elarbi M, Bechikh S, Ben Said L, et al. Multi-objective optimization: classical and evolutionary approaches[M]//Recent advances in evolutionary multi-objective optimization. Springer, Cham, 2017: 1-30.
\bibitem{b5} Haimes Y Y. Integrated system identification and optimization[M]//Control and Dynamic Systems. Academic Press, 1973, 10: 435-518.
\bibitem{b6} Dubey P. Inefficiency of Nash equilibria[J]. Mathematics of Operations Research, 1986, 11(1): 1-8.
\bibitem{b7} Yang Z, Bose A, Zhong H, et al. LMP revisited: A linear model for the loss-embedded LMP[J]. IEEE Transactions on Power Systems, 2017, 32(5): 4080-4090.
\bibitem{b8} Fan J Y, Zhang L. Real-time economic dispatch with line flow and emission constraints using quadratic programming[J]. IEEE Transactions on Power Systems, 1998, 13(2): 320-325.
\bibitem{b9} Lin Y, Johnson J X, Mathieu J L. Emissions impacts of using energy storage for power system reserves[J]. Applied energy, 2016, 168: 444-456.
\bibitem{b10} Mondal M A H, Mathur J, Denich M. Impacts of CO2 emission constraints on technology selection and energy resources for power generation in Bangladesh[J]. Energy Policy, 2011, 39(4): 2043-2050.
\bibitem{b11} Shin H, Kim T H, Kim H, et al. Environmental shutdown of coal-fired generators for greenhouse gas reduction: A case study of South Korea[J]. Applied Energy, 2019, 252: 113453.
\bibitem{b12} Granelli G P, Montagna M, Pasini G L, et al. Emission constrained dynamic dispatch[J]. Electric Power Systems Research, 1992, 24(1): 55-64.
\bibitem{b13} Koltsaklis N E, Georgiadis M C. A multi-period, multi-regional generation expansion planning model incorporating unit commitment constraints[J]. Applied energy, 2015, 158: 310-331.
\bibitem{b14} Shao C, Ding Y, Wang J. A low-carbon economic dispatch model incorporated with consumption-side emission penalty scheme[J]. Applied Energy, 2019, 238: 1084-1092.
\bibitem{b15} Eriksen P B. Economic and environmental dispatch of power/CHP production systems[J]. Electric Power Systems Research, 2001, 57(1): 33-39.
\bibitem{b16} Olsen D J, Dvorkin Y, Fernandez-Blanco R, et al. Optimal carbon taxes for emissions targets in the electricity sector[J]. IEEE Transactions on Power Systems, 2018, 33(6): 5892-5901.
\bibitem{b17} Wang Y, Qiu J, Tao Y, et al. Carbon-oriented operational planning in coupled electricity and emission trading markets[J]. IEEE Transactions on Power Systems, 2020, 35(4): 3145-3157.
\bibitem{b18} Gu N, Wang H, Zhang J, et al. Bridging Chance-constrained and Robust Optimization in an Emission-aware Economic Dispatch with Energy Storage[J]. IEEE Transactions on Power Systems, 2021, 37(2): 1078-1090.
\bibitem{b19} Lu Z, Liu M, Shang N, et al. Two-stage clearing model for day-ahead electricity market considering impact of carbon emissions trading markect[J]. Automation of Electric Power Systems, 2022, 46(10): 159-170. (in Chinese)
\bibitem{b20} Wang Y, Gong Y, Wang C, et al. Medium and long-term power purchase plan based on bargaining game[J]. Proceedings of the CSU-EPSA, 2013, 25(02): 136-142. (in Chinese)
\bibitem{b21} Wei W, Wang J, Mei S. Convexification of the nash bargaining based environmental-economic dispatch[J]. IEEE Transactions on Power Systems, 2016, 31(6): 5208-5209.
\bibitem{b22} Nash Jr J F. The bargaining problem[J]. Econometrica: Journal of the econometric society, 1950: 155-162.
\bibitem{b23} Borrelli F, Bemporad A, Morari M. Geometric algorithm for multiparametric linear programming[J]. Journal of optimization theory and applications, 2003, 118(3): 515-540.
\bibitem{b24} Chen Baolin. Optimization theory and algorithms (2nd Edition)[M]. Tsinghua University Press, 2005, 10: 143-145. (in Chinese)
\bibitem{b25} National Renewable Energy Laboratory (NREL) . Geospatial Data Science. https://www.nrel.gov/gis/
\bibitem{b26} World Bank. 2022. State and Trends of Carbon Pricing 2022. State and Trends of Carbon Pricing;. Washington, DC: World Bank. © World Bank. https://openknowledge.worldbank.org/handle/10986/37455 License: CC BY 3.0 IGO.
\end{thebibliography}

\fi
